Multi-dimensional discrimination in Law and Machine Learning -- A comparative overview

AI-driven decision-making can lead to discrimination against certain individuals or social groups based on protected characteristics/attributes such as race, gender, or age. The domain of fairness-aware machine learning focuses on methods and algorithms for understanding, mitigating, and accounting for bias in AI/ML models. Still, thus far, the vast majority of the proposed methods assess fairness based on a single protected attribute, e.g. only gender or race. In reality, though, human identities are multi-dimensional, and discrimination can occur based on more than one protected characteristic, leading to the so-called ``multi-dimensional discrimination'' or ``multi-dimensional fairness'' problem. While well-elaborated in legal literature, the multi-dimensionality of discrimination is less explored in the machine learning community. Recent approaches in this direction mainly follow the so-called intersectional fairness definition from the legal domain, whereas other notions like additive and sequential discrimination are less studied or not considered thus far. In this work, we overview the different definitions of multi-dimensional discrimination/fairness in the legal domain as well as how they have been transferred/ operationalized (if) in the fairness-aware machine learning domain. By juxtaposing these two domains, we draw the connections, identify the limitations, and point out open research directions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> checklist.tex <==
Check again
---------------------

--> Check again: sparsity is the wrong term, needs to be replaced with scarcity


--> discriminative vs discriminatory vs discriminating: which term should be used when?

--> Law: should be written in capital? (No)

--> Multi-dimensional/multi-dimensionality or multidimensional/multidimensionality? Same goes for sub-group/subgroup. Opinion Jan: I would go for the version without - because that's what people search for.

    
--> Court cases are now cited in footnotes. Is there a good way to add them as references instead?

--> quotation marks: `` ''

--> independent and identically distributed (i.i.d.)

use:  i.e.,
use: e.g., instead of e.g. or eg. or eg 

criterion or criteria?




Tasks (20/1/2023)
=========================
-> Clean the orphan inline comments
Arjun --> Eirini --> Jan
--> Eirini Section 4 (add example of "life discrimination"
--> Jan update the example (Arjun sends the paper)
--> Reduce the images
--> Improve Figure 3
--> Arjun re-check section 3 


todo: a new title
- Multi-dimensional discrimination - An overview
- Multi-dimensional discrimination in Law and ML
- Connecting Multi-dimensional discrimination in ML to its Legal counterpart
- Multi-dimensional fairness in law and machine learning - A comparative overview
//I like this

Question: Do you think it's a problem that we cite German literature? Not for anonymity but for the substantial review.

todo FORMALITIES
- Spelling and grammar: DONE
- Anonymisation: DONE
- References: DONE

todo: 1 - Shorten intro a little bit
DONE! Title+Abstract+Intro --> 2 pages
@Jan/Arjun: proof read

I also reduced a bit in Section 3, except for 3.4


todo: 2
Rephrase text for sequential example. DONE
Move figure 3 to the appropriate place in sec. 3 EDIT 06/02: With the new changes may stay at the current place.

todo: 3
Arjun: modify figure (data scarcity in ADULT: add positive/negative for Old White Male); take out papers on regression & counterfactuals; check & possibly remove par. on pufferfish privacy
Jan: read through sec. 3 and check intelligibility and consistency DONE until 3.3

todo: 4 - 4.1: Move to swh. else (intro) as a "disclaimer" and compress. DONE
4.2 (now 4.1): add sentence that connects issue with multi-dimensionality. DONE
4.3 (now 4.2): Boil down to key messages.DONE (as good as possible)


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> temp.tex <==


The term intersection in `intersectional discrimination' refers to the intersection of groups called sub-groups as defined in Eq. \ref{eq:sg}. Although, \cite{pmlr-multicalibration} was the first to study the fairness problem for finer sub-populations with their term of `multi-calibration', but \cite{kearns2018gerrymandering} was the first to explicitly study the problem on intersection of groups a.k.a. sub-groups in the ML literature. Any formal definition of cumulative discrimination as defined in Eq.~\ref{eq:genMF} can be adapted over different subgroups to define intersectional discrimination as follows:
\begin{equation}\label{eq:genIF}
    \mathcal{F}_S\equiv P(\hat{y}\mid {sg}_j,C)-P(\hat{y}\mid {sg}_i,C), \forall {sg}_j,{sg}_i \in \mathcal{SG}
\end{equation}

Since, intersectional discrimination is the most vividly studied multi-dimensional discrimination type in ML literature, we hereafter present a more detailed study of the most popular proposed ideas to measure intersection discrimination.

\subsubsection{\textbf{Statistical Parity Subgroup Fairness (SPSF)~\cite{kearns2018gerrymandering}:}}
Kearn et al.~\cite{kearns2018gerrymandering} argued
that any group fairness notion 
%addressing \mf~may still discriminate some fine-grained set of subgroups $sg \in SG$.
might appear to be equitable when 
considering either protected attribute alone, e.g., only gender or race, but might be unfair when looking at the intersection of different protected attributes
(e.g., black women).
Therefore, they extended  \emph{Statistical Parity} (SP)~\cite{dwork2012fairness_parity}  for \mf~ and introduced  \emph{Statistical Parity Subgroup Fairness} (\emph{SPSF}). 
%\todo{still you need to explain a bit what the formula is}
The idea is that the difference between the acceptance rate (probability of positive prediction) of any subgroup ${sg} \in SG$ ($\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+|{sg})$) 
from the overall acceptance rate ($\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+)$)  proportional to the relative size of the subgroup ($\mathbf{P}({sg})$) in the data, must be less than an allowed discrimination threshold $\epsilon$. 
More formally:
%The \mf~constraints $C_\mathcal{SG}$ are formulated as:
\begin{equation}
    \begin{split}
      \mathbf{P}({sg})\times\Big|\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+)-\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+|{sg})\Big|\leq \epsilon,~\forall {sg} \in \mathcal{SG} 
    \end{split}
\end{equation}
The threshold $\epsilon\in [0,1]$ quantifies the amount of allowed unfairness towards any subgroup $sg\in \mathcal{SG}$. The relative size of the subgroup ($\mathbf{P}({sg})$) allows to ignore forcing fairness criteria to small fractions of the population (subgroups which are very small in size e.g., a singleton subgroup) to avoid fairness overfitting. \emph{SPSF} being an adaptation of SP, ignores the ground truth labels and only considers model predictions~\cite{hardt2016equality}. 


The advantage of the fairness criteria lies in scenarios where a sub-group ${sg}$ is underrepresented in the positive class (like Black Females in Fig.~\ref{fig:toysankey}) because it allows to promote the underrepresented sub-group. 
The assumed scenario is highly likely when %sub-groups are defined over the intersection of a large 
the number of protected attributes is large. 

However, in absence of such an extreme scenario, a major drawback of the method is the possibility of high false positive rates e.g., higher chance of accepting unqualified members of a subgroup in order to balance the acceptance rate among the different sub-groups. Further, the method relies upon the subgroup probability  $\mathbf{P}(sg)$ estimated from the dataset and is therefore prone to biased data representations.

%in the dataset if any subgroup ${sg}$ has very low representation, then the quantified discrimination is also very low irrespective of actual discriminatory outcome of $\mathcal{M}$. 
%\color{red} Pros and cons \color{black}




\subsubsection{\textbf{False Positive Subgroup Fairness (FPSF)~\cite{kearns2018gerrymandering}:}}
The \mf~criteria for the widely used \snf~notion \emph{Equal Opportunity} (Eq.Opps)~\cite{hardt2016equality} on subgroups have been termed as \emph{False Positive (FP) Subgroup Fairness} (\emph{FPSF}). The constraint $C_\mathcal{SG}$ is based on the difference between incorrect acceptance (false positive) on a given sub-group ${sg}$ and incorrect acceptance on the entire population (dataset) proportional to relative size of the subgroup labelled as negative in the dataset, to be less than a given discrimination threshold. It is formulated as: 
\begin{equation}
    \begin{split}
        \mathbf{P}(Y=-,{sg})\times\Big|\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+|Y=-)-\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+|Y=-,{sg})\Big|\leq \epsilon,\\\forall {sg} \in \mathcal{SG} 
    \end{split}
\end{equation}
%For solving the constrained learning problem they used the two-player zero sum game (Minimax), where they termed the constraints $C_\mathcal{SG}$ as the agent Auditor and the training loss $l(X,\theta)$ as agent learner. Their solution approach is to find the equilibrium of this game. 

By considering ground truth labels, \emph{FPSF} overcomes the possibility of high false positives rates. However, like \emph{SPSF} they rely upon distribution of the subgroups, specifically in the negative (-) class. This has been criticized by
\cite{foulds2020intersectional} in their work, where they argue that the concept of subgroup fairness method 
due to the consideration of the probability of subgroup distribution $\mathbf{P}(Y=-,{sg})$, gets affected by the population size of the subgroup $|{sg}|$. Thus, a discrimination towards a subgroup ${sg}$ with a small population size gets unfairly overlooked.

Working on the similar principle, subgroup fairness has been further imposed on calibration criteria as multi-calibrations~\cite{hebert2018multicalibration} to ensure equlity in calibrated probability estimates among the subgroups.
%\color{red} Pros and cons \color{black}


\subsubsection{\textbf{Differential Fairness (DF)~\cite{foulds2020intersectional}:}}
Foulds et al.~\cite{foulds2020intersectional} in their work criticized the concept of subgroup fairness for its inability to tackle disproportionate distribution of subgroups. 
%They argued that the subgroup fairness definition~\cite{kearns2018gerrymandering} due to the consideration of the probability of subgroup distribution $\mathbf{P}({sg})$, gets affected by the population size of the subgroup $|{sg}|$. Thus, a discrimination towards a subgroup ${sg}$ with a small population size gets unfairly overlooked. 
To address the problem in hand they proposed the \mf~notion \emph{Differential Fairness} (DF)which extends the 80\%~\cite{equal1978guide} rule of `Equal Employment Opportunity Commission' to the multiple intersectional sub-groups case. The idea here is to restrict ratios of outcome probabilities
between groups under a predetermined fairness
threshold. The threshold is determined on a sliding scale which is inspired from a
definition of privacy for data-driven algorithms called \emph{differential privacy}~\cite{dwork2014privacy}.
which is formulated as:
\begin{equation}
    \begin{split}
        e^{-\epsilon}\leq\frac{\mathbf{P}(M(U,\mathcal{S})=y|{sg}_k)}{\mathbf{P}(M(U,\mathcal{S})=y|{sg}_m)}\leq e^{\epsilon},~~
        \forall {sg}_k,{sg}_m \in \mathcal{SG},k\neq m
    \end{split}
\end{equation}
Where $\epsilon$ is a small admissible discrimination towards any subgroup. For strict fairness equality $\epsilon$ is considered to be $0$.
\cite{foulds2020intersectional} in their work proved that the \emph{DF} definition guarantees fairness protections for all the underlying subgroups of the protected attributes,  making it consistent with the ethical principles of intersectionality theory.
The fairness criteria further provides privacy and economic guarantees which determine the fairness consequences for a given tolerance bound  $\epsilon$.

The fairness criteria is however, explicitly designed to extend the 80\% rule~\cite{equal1978guide} between any two sub-groups,  which identifies
disparate impact in cases where $P(y|{sg}_k)/P(y|{sg}_m) \leq 0.8$, for a disadvantaged subgroup ${sg}_k$, and best performing subgroup ${sg}_m$. Thus, restricting its adoption to other group fairness criteria~\cite{dwork2012fairness_parity,hardt2016equality,pleiss2017calibration}.

\subsubsection{Empirical differential fairness (EDF)~\cite{foulds2020intersectional}:}
The \emph{DF} criteria prerequisites $\mathbf{P}(M(U,\mathcal{S})=y|{sg}_k)$ to be known for all the defined subgroups ${sg}_k$. Thus, in cases where $\mathbf{P}(M(U,\mathcal{S})=y|{sg}_k)$ is unknown, ~\cite{foulds2020intersectional} suggested an alternative using the empirical distribution of the data. Under the assumption $P(y|g^i)=\frac{N_{y,g^i}}{N_{g^i}}$, where $N_{y,g^i}$ and $N_{g^i}$ are empirical counts of a group $g^i$ (a group defined by protected attribute $S|i|$) in class $y$ and empirical counts of the entire group $g^i$ population in the dataset respectively, \emph{EDF} is defined as: 
\begin{equation}
    \begin{split}
        e^{-\epsilon}\leq\frac{N_{y,g^j}}{N_{g^j}} \frac{N_{g^m}}{N_{y,g^m}}\leq e^{\epsilon},~~
        \forall {g}_j,{g}_m \in \mathcal{S},j\neq m
    \end{split}
\end{equation}

The \emph{EDF} criteria have the possibility of being unstable in extreme cases when almost all instances belongs to the same class. To overcome the challenge ~\cite{foulds2020intersectional} further proposed an alternative that uses soft counts for \emph{EDF}, based on the prediction of a probabilistic classifier. 

In a follow up work \cite{foulds2020bayesian} suggested a Bayesian modelling of the probabilistic classifier that generalizes $P(y|g^i)$ estimation beyond the available data, while reducing variance in estimation. A notable mention,  \cite{yang2020counterfactual_fairness} extended the idea of intersectional fairness using causal modelling and counterfactual instance generations, into the fair-ranking problem set-up, which is beyond the scope of this paper.


\begin{table}[]\caption{Summary of the intersectional fairness methodologies}\label{tab:intersectional}
\begin{tabular}{|l|l|l|l|}
\textbf{Method} & ~~~~~\textbf{Formulation} & ~~~~~~~~~~~~~~~~~~~~\textbf{Usability} \\ \hline
    SPSF~\cite{kearns2018gerrymandering}   &   \scriptsize \begin{tabular}[c]{@{}l@{}}$\mathbf{P}({sg}_j)\times\Big|\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+)-$\\ $\mathbf{P}(\mathcal{M}(U,\mathcal{S})=+|{sg}_j)\Big|\leq \epsilon$,\\ $\forall {sg}_j \in \mathcal{SG}$\end{tabular} \normalsize                 &      \begin{tabular}[c]{@{}l@{}}Advantageous where the positive representation \\ of any sub-group ${sg}_j$ is almost non-existent\end{tabular}                        \\
    FPSF~\cite{kearns2018gerrymandering} &                      &                             \\
   DF~\cite{foulds2020intersectional}    &                      &                             \\
  EDF~\cite{foulds2020intersectional}  &                      &                             \\ \hline
\end{tabular}
\end{table}


==> venues.tex <==


https://dl.acm.org/journal/jrc


https://www.springer.com/journal/43681
